Securing Monolithic Kernels using Compartmentalization

Monolithic operating systems, where all kernel functionality resides in a single, shared address space, are the foundation of most mainstream computer systems. However, a single flaw, even in a non-essential part of the kernel (e.g., device drivers), can cause the entire operating system to fall under an attacker's control. Kernel hardening techniques might prevent certain types of vulnerabilities, but they fail to address a fundamental weakness: the lack of intra-kernel security that safely isolates different parts of the kernel. We survey kernel compartmentalization techniques that define and enforce intra-kernel boundaries and propose a taxonomy that allows the community to compare and discuss future work. We also identify factors that complicate comparisons among compartmentalized systems, suggest new ways to compare future approaches with existing work meaningfully, and discuss emerging research directions.

==> applications.tex <==
\notetp{Discuss how they are used, probably linking to categories.}

\notedme{How do we want to relate this to the earlier evaluation section? I've put initial text there for now.}

\subsection{Confidentiality}

\subsection{Integrity}

\subsection{Availability}


==> categorisation.tex <==
\begin{table*}[t]
	\caption{Categorisation of each compartmentalization mechanisms implementation, along with the trust assumptions inferred from their threat model. We use \CIRCLE when the categorisation is clear, and \LEFTcircle when papers fit into more than one category}
\setlength\tabcolsep{5 pt}
	\begin{tabular}{|c||c|c|c|c||c|c|c|c|c|}
	  \hline
	  & \multicolumn{4}{c||}{\textbf{Compartmentalization Mechanism}} & \multicolumn{5}{c|}{\textbf{Stack View}\notenr{TODO - more descriptive name}}\\
	  \hline
	  \textbf{Paper} & Enclave & Exclave & Isolated Component & Nested Kernel & Traditional & Enclave & Exclave & Trusted Path & TrustZone\\
	  \hline
	  PerspicuOS~\cite{dautenhahn2015nested} &  &  &  & \CIRCLE &  & \CIRCLE &  &  & \\
	  \hline
	  MaKC~\cite{achermann2017separating} & \LEFTcircle &  & \LEFTcircle &  & \CIRCLE &  &  &  &\\
	  \hline
	  Nooks~\cite{swift2003improving} &  &  & \CIRCLE &  & \CIRCLE &  &  &  & \\
	  \hline
	  LVDs~\cite{narayanan2020lightweight} &  &  & \CIRCLE &  &  &  & \CIRCLE &  & \\
	  \hline
	  LXDs~\cite{Narayanan2019} &  & \CIRCLE &  &  &  &  & \CIRCLE &  & \\
	  \hline
	  KCoFI~\cite{criswell2014kcofi} &  &  & \CIRCLE &  & \CIRCLE &  &  &  & \\
	  \hline
	  \textsc{Kenali}~\cite{song2016enforcing} &  &  & \CIRCLE &  & \CIRCLE &  &  &  & \\
	  \hline
	  SVA Extensions~\cite{criswell_secure_2007,criswell_memory_2009} &  &  & \CIRCLE &  &  &  & \CIRCLE &  & \\
	  \hline
	  SKEE~\cite{azab_skee_2016} & \CIRCLE &  &  &  & \LEFTcircle &  &  &  & \LEFTcircle\\
	  \hline
	  LXFI~\cite{mao_software_2011} &  & \CIRCLE &  &  &  & \CIRCLE &  &  & \\
	  \hline
	  %
	 %
	  %
	  %
	\end{tabular}
\end{table*}

\subsection{Categories\notenr{Feel free to change}}
\label{sec:categories}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{./img/isolation-types.pdf}
	\caption{\notetp{todo caption.}}
	\label{img:isolation-types}
\end{figure}

	Compartmentalization mechanisms are techniques used for isolating the components\notevk{sub-systems a better word?}\notenr{Depends on how prescriptive we want to be, subsystem is quite specific to an area of the OS e.g. MMU, in theory you could isolate a component across multiple subsystems - e.g. a component with it's own MMU and Networking subsystem?}
	\notetp{are they really techniques? here we discuss more ways to attack the problem at high abstract level. How should we formulate this?}
	 of an  OS (at the Kernel level) from each other. This is beneficial as it reduces the impact and availability of attack vectors within a commodity o.s kernel.
	\subsubsection{Enclave}
		An enclave based compartmentalization scheme is characterised by its distrust of the core-kernel, with each of the sub-components in the kernel isolated in their own protection domain.
		\notetp{This is for example the approach taken in SKEE~\cite{} which isolate ...}

	\subsubsection{Nested Kernel}
		A nested kernel can be thought of as a special case of enclave as it has the core property of distrusting the core Kernel. Where we draw the distinction between an enclave and nested kernel is the granularity of the isolation. In this scheme, whole sub-systems of the kernel (e.g. the MMU) are virtualised and hidden from the core kernel, instead being managed by an inner-kernel that forms a greatly reduced TCB. This nested kernel will commonly expose a virtual api (e.g. vMMU) that the outer kernel can interact with to retain control over tasks like memory allocation. However it is the inner-kernel that will actually interact with the MMU (pMMU) after checking that the Kernels resource request does not violate a pre-defined security property.
		\notetp{ok is it not that we move the core kernel inside its own domain(s) separated from the non-core stuff? What do people think?}

	\subsubsection{Exclave}
		An exclave is the inverse of an enclave in that the core kernel is assumed to be trusted, will other components are modelled as untrusted (e.g. a device driver). In these isolation mechanisms, it is common to see security architectures that design a new kind of interface or interaction paradigm between the core-trusted kernel and the untrusted components.
		\notetp{This the approach taken, for example, in LXD~\cite{} which isolate xxx to yyy.}

	\subsubsection{Isolated Component}
		In our taxonomy, isolated components form a half-way point between enclave and exclave based mechanisms. They implemented an enclave based isolation scheme that isolates sub-components of a system from each other, and then using design principles from exclave based methods to provide a secure interface/interaction channel between this coarse-grained kernel components.
		This can be though as kernel composed of multi-distrustful subcomponents.
		\notetp{For example, Nooks~\cite{} ...}

\subsection{Separations of Trust}
\label{sec:stack-trust}

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{./img/isolation-types2.pdf}
	\caption{\notetp{todo caption.}}
	\label{img:isolation-types2}
\end{figure}

Having discussed the isolation categories in section \ref{sec:categories}, we
now discuss how this translates to separations of trust between isolated
components as shown in figure \ref{img:isolation-types2}.

\subsubsection{Horizontal Compartmentalization}
\label{subsubsec:traditional_stack}
A traditional approach to isolation closely resembles the textbook model of OS structuring that has an untrusted user-space and a trusted kernel.
Although the trusted kernel is assumed not be malicious, it may still be buggy.
For kernel isolation this translates to an untrusted area of Kernel space, that passes all requests for hardware resources via the trusted kernel
space.\notedok{Hmm, its a bit unclear what you are getting at here - maybe a
better name is needed than traditional.} The purpose of such isolation is to defend the kernel against attacks from user space, thereby improving the reliability of the kernel.
\notesyl{For example, KCoFI protects the OS from control flow-hijack attacks, return-to-user attacks, and code segment modification attacks; \textsc{Kenali} defend against memory-corruption based privilege escalation attacks. They both assumed the kernel not to be malicious, though it may be buggy.}
\notetp{I think we need to discuss that one.} \notesyl{do you mean make it clear that trusted kernel can also be buggy?}

\subsubsection{Vertical Compartmentalization}
\label{subsubsec:vertical}
Vertical Compartmentalization isolation separates the kernel into two separate execution environments (worlds): the normal (untrusted) world, and the secure (trusted) world. Transitions between these two worlds depends on a complete context switch, e.g. memory pages and peripherals are completely hidden from the normal world and are only accessible from/via the secure world.
For an instance, SKEE~\cite{azab_skee_2016} created an isolated lightweight execution environment with protected address space at the same privilege level of the kernel preventing the kernel from managing its memory translation tables and ensuring that switching from the OS Kernel to SKEE passes through a well-controlled switch gate.
\notetp{should we mention ARM trustzone here?}

\subsubsection{Enclave}\notetp{TODO: find a different name.}
In an enclave approach, critical kernel subsystems
are isolated and protected from the rest of the kernel/user space. The
majority of the kernel is designated as untrusted, instead opting to reduce
the TCB into a series of smaller isolated areas/components. Such isolation
uses a threat model in which the enclave is trusted but nothing outside of it, including the OS or any hypervisor, can be trusted. The reduced TCB allows finer-grained security policies to be enforced. For instance, the MMU subsystem may be entirely isolated from the kernel via a nested-kernel that performs management operations on behalf of the trusted kernel.

\subsubsection{Exclave}\notetp{TODO: find a different name.}
An exclave model takes the inverse of the enclave approach, compartmentalizing the kernel into a series of untrusted areas that are isolated from the trusted kernel. In contrast to the Traditional approach in Section \ref{subsubsec:traditional_stack} where the aim is to defend the kernel against attacks originating from the user space, an exclave aims to confine the effects of exploits to individual kernel subsystems. Although both approaches trusts the kernel to a certain extent, there is no clear separation of trust between the user space and the kernel space in the exclave model. An example here would be system extensions such as device drivers that have the capacity to crash the kernel. It is worth noting that an exclave model will not necessarily consider these isolated regions as malicious, but they do generally consider them 'buggy'. \notesyl{LXD supports isolation of device drivers which account for over millions lines of unsafe kernel code; LVDs are designed to block adversaries exploiting vulnerabilities in one of the kernel subsystems from attacking the rest of the kernel; Nooks provides a reliability layer intended to prevent driver-caused crashes, thereby improving the fault tolerance in OS. Similar to the assumptions made in the Traditional approach, they assume the kernel to be benign.}

\subsubsection{Trusted Path}
A trusted path can be thought of as a close relative to an enclave approach, again making the design decision to consider the kernel as untrusted.
A trusted path approach attempts to construct a direct path from the isolated component down to the hardware, without having to pass through another trusted component, or requiring a completely trusted kernel.
In theory, this ensures that any data communicated over trusted paths cannot be intercepted or modified by untrusted processes.



\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{img/part_mechs.png}
	\caption{Figure showing visualisation of compartmentalization mechanism categories\notenr{This is just a brain dump figure, and is by no means final}}
	\label{fig:kernel-part-approaches}
\end{figure}


==> future.tex <==
\notedok{Add section on whether some exclave techniques could be
revisited/reused for enclave and vice-versa.}
\notedok{Should we remark on API integrity from LXFI.}
\subsection{Language-Based Isolation}

Modern systems languages, such as Rust, have been designed with issues like memory safety in mind.
Thus it may be possible in the future to have \compz enforced at the language level via a managed runtime and/or during compilation.
Redleaf~\cite{narayanan_redleaf_2019, narayanan_redleaf_2020}, for instance, leveraged Rust's ownership model (that ensures that only one object is using a memory reference at any given moment) to enforce isolation and cross-domain communications using Remote References (RRefs) and a microkernel design.
Such approaches are able to provide high levels of isolation in software with a limited performance overhead, without requiring intensive hardware modifications.
We note that there has been a push for the adoption of Rust in the Linux kernel~\cite{rust_lwn}, notably including Google.
What could be accomplished in the context of an existing monolithic OS written in C remains to be explored.
\notedok{Could we argue that better tool support is needed for migrating
existing C code to Rust? Also that more work is needed to understand what might
constitue 'idiomatic' Rust in the Linux kernel and how that might differ from
user-space Rust code}

\subsection{New Hardware Mechanisms}

\mypar{Tagged Memory}
Intel Memory Protection Keys~(MPK) provide a mechanism for grouping memory pages into
one of 16 protection domains. Hardware ISA extensions allow the CPU to track
page accesses and trigger a fault if a domain tries to access a page
belonging to another domain. MPK has been used in a unikernel context for providing
intra-unikernel isolation to partition library operating systems into trusted and
untrusted regions \cite{sung_intra-unikernel_2020,sartakov21}.

Ahead of Intel's Trust Domain eXtensions (TDX) and support for supervisor
protection keys (SPK) \cite{PKSPMEMAdd}, \notesid{Moved IskiOS to MPK section}IskiOS~\cite{iskios_raid_21} demonstrates an
unconventional methodology for providing such protections by treating all of
system memory as user-space memory and reserving 8 protection keys for the
kernel. However in the absence of a hardware tagged memory system, IskiOS must
share the limited number of protection keys with user-space. Manipulation of the
user-space/kernel-space boundary may also result in side-channel attacks.

We can see a use-case for hardware-supported versions for this style of kernel
\compzz, such as assigning each device driver to a separate protection domain in
an exclave model. Existing hardware such as Intel MPK suffers from limited
domain scalability and mono-domain membership (a page can only be part of one
protection domain at a time). However recent work on RISC-V overcomes both
limitations~\cite{delshadtehrani_efficient_2020,schrammel_donky_2020},
potentially making them an even more viable kernel \compz mechanism in the future. 

\mypar{CHERI}
CHERI is a novel approach to \compz that embeds capability management and operations in the hardware as an ISA extension for RISC~\cite{woodruff_cheri_2014,watson_cheri_2015}, and more recently ARM-v8~\cite{morello,morello2}.
It provides spacial memory safety out of the box, and can also be extended to provide temporal safety~\cite{wesley_filardo_cornucopia_2020} like previous hardware approaches.
To date, much of the focus has been on user-space application partitioning.
However, there is no fundamental barrier to using CHERI in the context of kernel
\compzz.

\subsection{Deconflating Boundary Policies from Mechanism}

Past papers have studied the identification and expression of boundary policies~\autoref{sec:boundaries} in conjunction with the mechanism to provide isolation~\autoref{sec:mechanisms} often conflating the two.
FlexOS~\cite{lefeuvre2021flexos} expresses \compz policies through a combination of code annotation and IDL (see \autoref{sec:boundaries}).
Developers specify a series of call-gate, memory isolation,
and other \compz mechanisms as functions that are automatically inserted during compilation as appropriate.
The authors demonstrate the effectiveness of the approach by implementing from
the same policies both MPK- and VM-based \compzz.
While the work is still at an early stage it could pave the way for practical mainstream \compz across different hardware architectures.
Once the policy is specified, supporting new architectures or \compz mechanisms only requires the implementation of a well-defined set of functions, although generalizability beyond the two provided examples remains to be demonstrated.
\notedok{Could we argue that more work is needed on formal modeling of what kind
of the security policies achieved by different compartmentalisation strategies?
For example, given we have some isolation mechanism with certain isolation
properties, how can we verify that a certain compartmentalisation strategy
achieves a given security property?}
\subsection{Hardware Vulnerabilities}

In recent years, a number of flaw in hardware design, particularly around speculative execution, have been uncovered~\cite{lipp2018meltdown,kocher2019spectre}.
Those flaws break confidentiality expectations by creating cache side-channel from where information can be leaked across memory domain boundaries.
Userspace TEEs, notably Intel SGX, have been shown to be susceptible to such vulnerabilities~\cite{chen2019sgxpectre,van2018foreshadow,koruyeh2018spectre}.
Effectively closing this attack channel is proving extremely difficult in practice as they are caused by a fundamental flaws in CPU designs that cannot be easily patched out~\cite{mcilroy2019spectre} and the implemented mitigations are the source of significant performance overhead (\ie up to 89\% for the poll operation)~\cite{ren2019analysis}.
These hardware vulnerabilities have only become apparent recently, and thus have not been addressed thoroughly yet in the kernel \compz literature.
Hardware vulnerabilities are orthogonal to kernel \compz techniques, but should be considered as part of the threat model when designing solutions that aim to provide confidentiality guarantees.

\notedok{There has been some work on making a more flexible/modular kernel in
the context of virtualized unikernels in order to improve performance through
specialization (e.g. unikraft), but
with some downsides (e.g. in terms of restricting the OS to single address space
applications). To what extent can the architectural lessons learned there be
applied to improve security in a more general setting (i.e. there is a need to support multiple
applications)?} 




==> threat.tex <==


Threat models describing assumptions
  made about the \emph{trusted components}, \emph{attack surface},
  and \emph{adversaries}
  influence the design of kernel compartmentalization.
In~\autoref{sec:threat:trust}, we categorize kernel \compz techniques into one of two broad \compz
strategies, \emph{exclave} and \emph{enclave}, to help
illustrate how trust
models influence the design space.
Exclaves \emph{prevent} a distrusted component from corrupting the rest of the
system; enclaves \emph{protect} a trusted component from the rest of the system.
In~\autoref{sec:threat:adversary}, we discuss the security goals of existing
work with respect to exclaves, enclaves and the confidentiality-integrity-availability~(CIA) triad.

\subsection{Trust Model}
\label{sec:threat:trust}

A trust model assigns different levels of trust to each component within a system, drawing a boundary between the untrusted components that are either buggy or malicious, and the trusted components that are assumed benign.
\autoref{img:partitioning_strategies} shows a simplified representation of the trust models for exclaves and enclaves.

\mypar{Exclaves} Exclave approaches generally assume that the kernel is benign, though it may contain bugs or vulnerabilities.
To confine the impact of exploits, exclave approaches compartmentalize the kernel into a set of untrusted domains where bugs or vulnerabilities are commonly found, ensuring that their effects are isolated.

For example, exclaves are suitable for isolating kernel extensions such as
device drivers, which have contributed to the majority of Linux kernel
vulnerabilities~\cite{chen2011linux,palix2011faults,linux_vulntrend}.  Exclaves
restrict kernel extensions' access to kernel memory and privileged instructions,
interposing on interactions between extensions and the core kernel to enforce
\emph{the principle of least privilege} (\eg LXFI, which restricts an
extension's access to memory and callback functions~\cite{mao_software_2011}).  
Similarly, vulnerabilities are also found in kernel subsystems such as file systems or
network stacks.
For example, a flaw (CVE-2020-27815) was discovered in the Linux JFS filesystem, allowing local attackers to cause system panic, memory corruption or privilege escalation~\cite{cve2020_27815}.
In the extreme, the kernel can be decomposed into \emph{multiple} mutually-distrusting exclave domains, each implementing a subset of kernel functionality, so that faults in a domain do not affect the functionality of other domains (\eg Sawmill~\cite{Smith1985} and VirtuOS~\cite{nikolaev_virtuos_2013}).

On the other hand, exclaves only protect the monolithic kernel from components
explicitly designated as less reliable. Vulnerabilities lurking outside the
exclaves remain a threat to the kernel and its security mechanisms. Indeed, a
vulnerability in one area of kernel functionality can open a path to
compromising a core kernel security mechanism.


\mypar{Enclaves} In contrast to exclaves, enclave approaches isolate trusted code instead of untrusted code.
Enclave approaches typically assume a trust model in which the kernel is not only assumed to contain vulnerabilities, but may also be acting maliciously under an attacker's control.
Therefore, enclaves are typically used for protecting critical kernel functionality, such as kernel protection and monitoring mechanisms.
Enclaves achieve this by isolating sensitive kernel functionalities from the rest of the kernel, and thereby minimizing their attack surface.
To create an isolated security domain, many enclave techniques~\cite{criswell2014kcofi,dautenhahn2015nested,song2016enforcing,azab_skee_2016} isolate the memory management unit (MMU),
giving exclusive control of the MMU to a
small trusted code section while mediating the MMU access provided to
the rest of the kernel.
This mediation allows protection of certain functionalities, for example, carving out a separate security domain to implement a tamper-proof logging mechanism~\cite{dautenhahn2015nested}.






\subsection{Security Goals}
\label{sec:threat:adversary}

It is important to understanding the types of attacks a mechanism aims to protect against.
In this section, we explore the security goals of kernel compartmentalization.
We model those goals with respect to the CIA triad and discuss the efficacy
of exclaves and enclaves in achieving those goals.




\mypar{Confidentiality}
A kernel provides confidentiality guarantees when it prevents an attacker from accessing protected or sensitive data from the kernel.
A compromised kernel represents an extremely high confidentiality risk as an attacker could gain access to sensitive information anywhere in the system and disclose this information (\eg leaking cryptographic keys).

Most exclave solutions focus on write protection rather than read protection.
As previously mentioned, they isolate less trusted kernel extensions from the rest of the kernel and control the \emph{write} operations extensions perform outside of their security domains.
Therefore as a matter of course, they tend to not provide confidentiality guarantees.
However, we note that certain exclaves such as SFI~\cite{sfi93}, Mondrix~\cite{witchel2005mondrix}, XFI~\cite{erlingsson2006xfi}, and BGI~\cite{castro2009fast} can control read operations.
This prevents a compromised extension running within an exclave from extracting secrets from the rest of the kernel.
However, this typically comes at the cost of slower overall execution.


As previously stated, enclave approaches generally isolate a protected address space from the rest of kernel, and restrict the wider kernel's access to the MMU so as to keep the enclaves secure.
By doing so, enclaves create a secure memory region that cannot be accessed by any of the untrusted parts of the kernel, hence guaranteeing the confidentiality of the data in that protected region.
For instance, SeCage~\cite{Liu2015} protects sensitive information (\eg cryptographic keys) from kernel memory disclosure by decomposing a monolithic system mechanism (\eg CryptoLoop) into secret compartments containing sensitive information and its corresponding code, and a main compartment where the rest of the mechanism logic resides.
Each compartment is assigned an isolated address space so as to restrict functions outside of the secret compartment from accessing the sensitive information in the enclave.


\mypar{Integrity}
Kernel integrity encompasses the property of being tamper-proof,
which requires the kernel to be protected from any
modifications that would cause an unexpected change in its behaviour~\cite{Biba1977}.
With the kernel being the TCB of most computer systems, kernel integrity is
fundamental to the trustworthiness of the whole system.

Common monolithic kernels are implemented using memory unsafe languages, and thus are %
vulnerable to memory corruption, which is a violation of
integrity that may lead to attacks such as privilege escalation, arbitrary code execution,
denial-of-service (DoS).
For example, a double free vulnerability in the
raw MIDI kernel driver can lead to elevated %
privileges~\cite{cve2018_10902}, and a heap-based buffer overflow in the Marvell
WiFi chip driver allows adversaries to
perform arbitrary code execution~\cite{cve2019_14814}. 
Adversaries can also
compromise kernel integrity to evade kernel defense mechanisms.  For example, an
integer overflow in Android exposes a TOCTOU condition that may be used to
bypass the Peripheral Image Loader (PIL) authentication~\cite{cve2016_8438}.

Exclave approaches encapsulate unreliable code within its own compartment, shielding the rest of the kernel from potential integrity threats.
By interposing on inter-domain interactions, one is able to restrict the privileges of exclaves, limiting an adversary's access to kernel resources so as to prevent unauthorized tampering.
For instance, LXFI~\cite{mao_software_2011}, LXDs~\cite{Narayanan2019}, and LVD~\cite{narayanan2020lightweight} confine the impact of kernel extensions by restricting the exclave's access to privileged operations.
Thus, if an attacker compromises an isolated component within the exclave, the attacker cannot misuse its escalated privilege to tamper with the rest of the kernel. 
As shown in \autoref{tab:decomposition},
\notedme{This shouldn't be the first reference to \autoref{tab:decomposition}}
Nooks, Mondrix and BGI do not explicitly state that they provide integrity guarantees and instead focus on availability.
However, they have the potential to provide integrity guarantees as they provide mechanisms to restrict write access.
Similarly while integrity is not the main focus of the papers, Microdrivers~\cite{ganapathy_microdrivers_2008} and Decaf~\cite{renzelmanndecaf} run their isolated compartments in userspace with no possibility to write to kernel address spaces, while VirtuOS~\cite{nikolaev_virtuos_2013} run them in fully separate VMs.

Conversely, enclaves provide an isolated memory space in which 
sensitive functionality can safely reside.
Since the protected memory region is inaccessible to the rest of the 
kernel, an
attacker exploiting vulnerabilities in the kernel is unable to tamper with the resources related to the isolated mechanisms.
For example, security mechanisms can be placed in enclaves to prevent defense bypass.
For instance, 
SKEE~\cite{azab_skee_2016} ensures that security tools are tamper-proof by executing them in an isolated environment that has total control over MMU modifications.
Enclaves have also been used as a means to increase overall system integrity, \eg
KCoFI~\cite{criswell2014kcofi} uses an enclave to guarantee that the critical data used by its Control Flow Integrity (CFI) mechanism cannot be tampered with.

\mypar{Availability}
Availability requires that a system, including its services and resources, can be used and accessed when needed.
However, a monolithic kernel has multiple points of failure
that could affect system availability.  As the entire monolithic kernel resides
in a single shared address space, any faults in the kernel may corrupt the
kernel and cause the system to crash.  In fact, over 50\% of the Linux
vulnerabilities reported in the past two decades lead to a kernel panic or
denial-of-service (DoS)~\cite{linux_vulntrend}. 
In our categorization (see \autoref{tab:decomposition}), we consider that a system provides availability guarantees if it implements some form of fault detection and/or recovery mechanism.

Exclaves improve system availability and reliability by confining the potential faults or vulnerabilities within 
kernel components.
For instance, VirtuOS~\cite{nikolaev_virtuos_2013} can survive crashes in
individual service compartments without adversely affecting the operation of other isolated compartments. 
Besides fault isolation, in systems such as Nooks~\cite{swift2003improving} exclaves are also able to facilitate fault detection by interposing and monitoring the inter-domain interactions for abnormal behaviours.
Once detected, recovery may be triggered immediately to minimize the impact on processes relying on the failing module.

On the contrary, enclaves are generally not designed to preserve system availability.  
Indeed, the goal of an enclave is to protect trusted and often security critical kernel components.
Consequently, a fault in an enclave is likely to adversely affect the entire system (\eg the entire security mechanism it protects may be rendered inoperative).%

